Chemodynamical modelling of the Milky Way

Chemodynamical models of our Galaxy that have analytic Extended Distribution Functions (EDFs) are likely to play a key role in extracting science from surveys in the era of Gaia.

==> macros.tex <==
%%%%% AUTHORS - PLACE YOUR OWN MACROS HERE %%%%%
\arraycolsep0.35mm                      % makes multiple equations look nice
\catcode`\@=11
\def\gta{\ifmmode{\,\mathrel{\mathpalette\@versim>\,}}
    \else{$\,\mathrel{\mathpalette\@versim>}\,$}\fi}
\def\lta{\ifmmode{\,\mathrel{\mathpalette\@versim<\,}}
    \else{$\,\mathrel{\mathpalette\@versim<}\,$}\fi}
\def\@versim#1#2{\lower 2.9truept \vbox{\baselineskip 0pt \lineskip
    0.5truept \ialign{$\m@th#1\hfil##\hfil$\crcr#2\crcr\sim\crcr}}}
\catcode`\@=12  
%%%%%%%%%%%%%%%%%%%
% My own definitions
\renewcommand{\[}{\begin{equation}}
\renewcommand{\]}{\end{equation}}
% Bold face Greek letters
%
\font\gkvecten=cmmib10
\font\gkvecseven=cmmib7
\let\boldgrk=\gkvecten
\let\boldgrksc=\gkvecseven

\def\gkthing#1{{\mathchoice%
	{\hbox{{\boldgrk\char#1}}}
	{\hbox{{\boldgrk\char#1}}}
	{\hbox{{\boldgrksc\char#1}}}
	{\hbox{{\boldgrksc\char#1}}}}}
\def\rms{{\sc rms}}
\def\valpha{\gkthing{11}}
\def\vbeta{\gkthing{12}}
\def\vgamma{\gkthing{13}}
\def\vdelta{\gkthing{14}}
\def\vepsilon{\gkthing{15}}
\def\vzeta{\gkthing{16}}
\def\veta{\gkthing{17}}
\def\vtheta{\gkthing{18}}
\def\viotaeta{\gkthing{19}}
\def\vkappa{\gkthing{20}}
\def\vlambda{\gkthing{21}}
\def\vmu{\gkthing{22}}
\def\vnu{\gkthing{23}}
\def\vxi{\gkthing{24}}
\def\vpi{\gkthing{25}}
\def\vrho{\gkthing{26}}
\def\vsigma{\gkthing{27}}
\def\vtau{\gkthing{28}}
\def\vupsilon{\gkthing{29}}
\def\vphi{\gkthing{30}}
\def\vchi{\gkthing{31}}
\def\vpsi{\gkthing{32}}
\def\vomega{\gkthing{33}}
{\newif\ifnotend
\notendtrue
\def\veclist{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz.}
\def\top#1#2.{#1}
\def\tail#1#2.{#2.}
\loop\expandafter\xdef\csname v\expandafter\top\veclist\endcsname%
{{\noexpand\bf\expandafter\top\veclist}}
\edef\veclist{\expandafter\tail\veclist}
\if\veclist.\notendfalse\fi\ifnotend\repeat}
{\newif\ifnotend
\notendtrue
\def\veclist{ABCDEFGHIJKLMNOPQRSTUVWXYZ.}
\def\top#1#2.{#1}
\def\tail#1#2.{#2.}
\loop\expandafter\xdef\csname c\expandafter\top\veclist\endcsname%
{{\noexpand\cal\expandafter\top\veclist}}
\edef\veclist{\expandafter\tail\veclist}
\if\veclist.\notendfalse\fi\ifnotend\repeat}
\def\amoeba{{\sc amoeba}}
\def\p{\partial}
\def\i{{\rm i}}
\def\df{{\sc df}}\def\edf{{\sc edf}}
\def\cE{{\cal E}}
\def\SN{S_{\rm N}}
\def\Teff{T_{\rm eff}}
\def\logg{\log g}
\def\feh{[{\rm Fe/H}]}\def\afe{[\alpha/{\rm Fe}]}
\def\vlos{v_{\rm los}}
\def\fracj#1#2{{\textstyle{#1\over#2}}}
\def\pa{\partial}
\def\ex#1{\left\langle#1\right\rangle}
\def\Rc{R_{\rm c}}\def\vc{v_{\rm c}}
\def\Rd{R_{\rm d}}
\def\Phic{\Phi_{\rm c}}
\def\Phieff{\Phi_{\rm eff}}
\def\mas{\,{\rm mas}}
\def\km{\,{\rm km}}
\def\cm{\,{\rm cm}}
\def\kms{\,{\rm km}\,{\rm s}^{-1}}
\def\mag{\,{\rm mag}}
\def\Myr{\,{\rm Myr}}
\def\yr{\,{\rm yr}}
\def\sec{\,{\rm s}}
\def\Gyr{\,{\rm Gyr}}
\def\K{\,{\rm K}} \let\kelvin=\K
\def\pc{\,{\rm pc}}
\def\kpc{\,{\rm kpc}}
\def\ergs{\,{\rm erg}}
\def\hi{H\,{\sc i}}
\def\e{{\rm e}}
\def\rd{{\rm d}}
\def\msun{\,{\rm M}_\odot}
\def\Lsun{\,{\rm L}_\odot}
\def\Fe{{\rm Fe}}
\def\meh{\hbox{[Me/H]}}
\def\feh{\hbox{[Fe/H]}}
\def\cafe{[\hbox{Ca}/\hbox{Fe}]}
\def\ofe{[\hbox{O}/\hbox{Fe}]}
\def\zeh{\hbox{[$Z$/H]}}
\def\alphaH{[\alpha/\hbox{H}]}
\def\afe{[\alpha/\hbox{Fe}]}
\def\HI{H\texttt{I}}
\def\dex{\,{\rm dex}}
\def\Rg{R_{\rm g}}
\def\vpbar{\overline{v}_\phi}
\def\figref#1{Fig.~\ref{#1}}
%%%%
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

%%%%%%
\def\rhodm{\rho_{\rm dm,\odot}}
\def\zthin{z_{\rm thn}}
\def\zthick{z_{\rm thk}}
\def\fthick{f_{\rm thk}}
\def\rd{{\rm d}}

